Relational Semantics for Databases and Predicate Calculus

The relational data model requires a theory of relations in which tuples are not only many-sorted, but can also have indexes that are not necessarily numerical. In this paper we develop such a theory and define operations on relations that are adequate for database use. The operations are similar to those of Codd's relational algebra, but differ in being based on a mathematically adequate theory of relations. The semantics of predicate calculus, being oriented toward the concept of satisfiability, is not suitable for relational databases. We develop an alternative semantics that assigns relations as meaning to formulas with free variables. This semantics makes the classical predicate calculus suitable as a query language for relational databases.

==> 10.further.tex <==
\section{Further work}\label{sec:fuWork}

The ``many-sorted logics'' presented
in \cite{ndr72,gllr86} are still intended on
interpretation by relations consisting of tuples
with numerical indexes.
This neither fills the requirements of databases
nor uses to the full the capabilities of \etr.
A suitable extension of the many sorted logics defined in 
\cite{ndr72,gllr86} is called for.

It is not to be expected
that the experts (mathematicians or logicians)
will do this work:
to them it is a trivial complication
of what is working fine in their area of interest.
It must be admitted that the extension from numerically-indexed,
single-sorted to many-sorted, arbitrarily indexed in the
\emph{language} of predicate calculus is not an enticing prospect;
a more abstract approach might be attractive.

It is the language that needs extension.
From an abstract point of view,
language is determined by an algebra,
the syntax algebra.
Meaning is a homeomorphism from the syntax algebra
to the semantic algebra
(a suitable formalization of \etr,
including filtering).
In an abstract formulation such as category theory,
Cartesian products need not be sets of tuples,
so the nature of the index set (numerical or not)
does not arise.
Moreover, in category theory the Cartesian product construction
is dual to the abstract version of the discriminated union of sets,
which we used to describe the types of many-sorted tuples.





